X-ray Spectral Survey of WGACAT Quasars, I: Spectral Evolution & Low Energy Cut-offs

We have used the WGA catalog of ROSAT PSPC X-ray sources to study the X-ray spectrum of about 500 quasars in the redshift interval 0.1--4.1, detected with a signal to noise better than 7. We have parameterized the PSPC spectrum in terms of two `effective energy spectral indices', alpha_Soft (0.1-0.8 keV), and alpha_Hard (0.4-2.4 keV), which allows for the different Galactic N_H along the quasars line of sight. We have used these data to explore the questions raised by the initial PSPC high redshift quasar studies, and in particular the occurrence of low X-ray energy cut-offs in high redshift radio-loud quasars. We have also studied the emission spectra of a large sample of radio-loud and radio-quiet quasars and studied their differences. We find that low energy X-ray cut-offs are more commonly (and perhaps exclusively) found in radio-loud quasars. Therefore the low energy X-ray cut-offs are physically associated with the quasars, and not with intervening systems, since those would affect radio-quiet and radio-loud equally. We suggest that photoelectric absorption is a likely origin of the these cut-offs.

==> README <==
%auto-ignore
README for:
	"X-ray Spectral Survey of WGACAT Quasars, I:
	Spectral Evolution \& Low Energy Cut-offs"
by
Fiore et al.,

Ap.J. paper #36319

directory includes:

README		--this file
reform.tex	--LaTeX file of paper including 6 Tables.
		  prepared using aasmacros
aaspp.sty	-- .sty file from aasmacros
f1.eps		--postscript file of figure 1
f2.eps		--postscript file of figure 2
f3a.eps		--postscript file of figure 3a
f3b.eps		--postscript file of figure 3b
f4.eps		--postscript file of figure 4
f5a.eps		--postscript file of figure 5a
f5b.eps		--postscript file of figure 5b
f6a.eps		--postscript file of figure 6a
f6b.eps		--postscript file of figure 6b
f7.eps		--postscript file of figure 7
f8.eps		--postscript file of figure 8


